Character-Aware Models Improve Visual Text Rendering

Current image generation models struggle to reliably produce well-formed visual text. In this paper, we investigate a key contributing factor: popular text-to-image models lack character-level input features, making it much harder to predict a word's visual makeup as a series of glyphs. To quantify this effect, we conduct a series of experiments comparing character-aware vs. character-blind text encoders. In the text-only domain, we find that character-aware models provide large gains on a novel spelling task (WikiSpell). Applying our learnings to the visual domain, we train a suite of image generation models, and show that character-aware variants outperform their character-blind counterparts across a range of novel text rendering tasks (our DrawText benchmark). Our models set a much higher state-of-the-art on visual spelling, with 30+ point accuracy gains over competitors on rare words, despite training on far fewer examples.

==> table-wikispell-results-all-langs-full.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabular}{@{}
                L{9mm}
                @{}
                L{16mm}
                @{\hspace{1mm}}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                @{\hspace{0.5mm}}
                R{3.5mm}
                @{\hspace{1.5mm}}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                R{3.5mm}
                @{\hspace{0.5mm}}
                R{3.5mm}
                @{}}
\toprule
\multicolumn{1}{c}{}                            
    & \multicolumn{1}{c}{}
    & \multicolumn{8}{c}{\textbf{mT5}}         
    & \multicolumn{8}{c}{\textbf{ByT5}}
\\ \cmidrule(lr){3-10} \cmidrule(lr){11-18} 
\multirow{-2}{*}{Size} 
  & \multirow{-2}{*}{\shortstack[c]{Frequency\\Bucket}}
  & ar
  & en
  & fi
  & ko
  & ru
  & th
  & zh
  & \textsc{avg}
  & ar
  & en
  & fi
  & ko
  & ru
  & th
  & zh
  & \textsc{avg}
\\ \midrule
Base
    & Top 1\%                        & \cellcolor[HTML]{E98F87}19 & \cellcolor[HTML]{E67D74}6  & \cellcolor[HTML]{E88880}14 & \cellcolor[HTML]{EDA49D}33 & \cellcolor[HTML]{E7837A}11 & \cellcolor[HTML]{F2BDB9}50 & \cellcolor[HTML]{F6D3D0}65 & \cellcolor[HTML]{EC9D96}28 & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{A7DCC2}97 & \cellcolor[HTML]{9BD7B9}98 & \cellcolor[HTML]{BCE4D1}97  & \cellcolor[HTML]{85CEAA}99  & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{8AD0AD}98 \\
    & 1--10\%                        & \cellcolor[HTML]{EA948C}22                      & \cellcolor[HTML]{E68178}9  & \cellcolor[HTML]{E7837B}11 & \cellcolor[HTML]{EEA7A1}35 & \cellcolor[HTML]{E67F76}8  & \cellcolor[HTML]{EB9890}25 & \cellcolor[HTML]{F8DEDB}72 & \cellcolor[HTML]{EB9A93}26 & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{9BD7B9}98 & \cellcolor[HTML]{9BD7B9}98 & \cellcolor[HTML]{79C9A2}99  & \cellcolor[HTML]{73C79E}99  & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{7AC9A3}99 \\
    & 10--20\%                       & \cellcolor[HTML]{EB9891}25                      & \cellcolor[HTML]{E67D74}7  & \cellcolor[HTML]{E7847B}11 & \cellcolor[HTML]{EFAEA9}40 & \cellcolor[HTML]{E68077}9  & \cellcolor[HTML]{E88B83}16 & \cellcolor[HTML]{FBEFEE}84 & \cellcolor[HTML]{EC9C95}27 & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{AADDC4}97 & \cellcolor[HTML]{A4DAC0}98 & \cellcolor[HTML]{61BF91}100 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{78C9A1}99 \\
    & 20--30\%                       & \cellcolor[HTML]{EB9790}25                      & \cellcolor[HTML]{E67C73}6  & \cellcolor[HTML]{E67E75}7  & \cellcolor[HTML]{EEAAA4}37 & \cellcolor[HTML]{E67F77}8  & \cellcolor[HTML]{EB9B94}27 & \cellcolor[HTML]{FBEEED}83 & \cellcolor[HTML]{EC9C95}28 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{A1D9BE}98 & \cellcolor[HTML]{A4DAC0}98 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{7FCCA6}99  & \cellcolor[HTML]{80CCA6}99 \\
   & Bottom 50\%                    & \cellcolor[HTML]{EA928B}21                      & \cellcolor[HTML]{E67C73}6  & \cellcolor[HTML]{E67D74}7  & \cellcolor[HTML]{F0B0AB}41 & \cellcolor[HTML]{E67F77}8  & \cellcolor[HTML]{EB9992}26 & \cellcolor[HTML]{FCEFEE}84 & \cellcolor[HTML]{EC9C95}28 & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{9ED8BB}98 & \cellcolor[HTML]{92D3B3}98 & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{61BF91}100 & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{78C9A1}99 \\
\midrule
Large
    & Top 1\%                        & \cellcolor[HTML]{F1B5B0}45                      & \cellcolor[HTML]{EC9C96}28 & \cellcolor[HTML]{EEA9A3}37 & \cellcolor[HTML]{EFAFA9}40 & \cellcolor[HTML]{EFABA5}38 & \cellcolor[HTML]{F3C5C1}55 & \cellcolor[HTML]{F8DCD9}71 & \cellcolor[HTML]{F1B5B0}45 & \cellcolor[HTML]{88CFAD}98  & \cellcolor[HTML]{B3E1CA}97 & \cellcolor[HTML]{B6E2CC}97 & \cellcolor[HTML]{98D5B7}98  & \cellcolor[HTML]{B0DFC8}97  & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{8ED2B1}98  & \cellcolor[HTML]{9AD6B9}98 \\
    & 1--10\%                        & \cellcolor[HTML]{F4CAC6}59                      & \cellcolor[HTML]{EEA8A2}36 & \cellcolor[HTML]{EEAAA4}37 & \cellcolor[HTML]{F3C1BC}53 & \cellcolor[HTML]{EEA9A3}37 & \cellcolor[HTML]{F0B1AC}42 & \cellcolor[HTML]{F8DDDB}72 & \cellcolor[HTML]{F1BAB5}48 & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{DEF2E8}96 & \cellcolor[HTML]{9ED8BB}98 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{A4DAC0}98  & \cellcolor[HTML]{A1D9BE}98  & \cellcolor[HTML]{79C9A2}99  & \cellcolor[HTML]{96D5B6}98 \\
    & 10--20\%                       & \cellcolor[HTML]{F7D5D3}67                      & \cellcolor[HTML]{EDA49E}33 & \cellcolor[HTML]{EEA8A3}36 & \cellcolor[HTML]{F6D3D0}65 & \cellcolor[HTML]{EFAFA9}40 & \cellcolor[HTML]{EB9A94}27 & \cellcolor[HTML]{FBEBEA}81 & \cellcolor[HTML]{F2BDB8}50 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{C2E7D5}97 & \cellcolor[HTML]{CFECDD}96 & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{82CDA8}99  & \cellcolor[HTML]{7FCCA6}99  & \cellcolor[HTML]{95D4B5}98  & \cellcolor[HTML]{92D3B4}98 \\
    & 20--30\%                       & \cellcolor[HTML]{F6D3D0}65                      & \cellcolor[HTML]{EDA49D}33 & \cellcolor[HTML]{EEA9A3}36 & \cellcolor[HTML]{F6D4D1}66 & \cellcolor[HTML]{F0B2AC}42 & \cellcolor[HTML]{F1B6B1}46 & \cellcolor[HTML]{FAE8E7}79 & \cellcolor[HTML]{F3C1BC}53 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{C2E7D5}97 & \cellcolor[HTML]{B6E2CC}97 & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{73C79E}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{7CCAA4}99  & \cellcolor[HTML]{85CEAA}99 \\
    & Bottom 50\%                    & \cellcolor[HTML]{F6D4D1}66                      & \cellcolor[HTML]{EDA39C}32 & \cellcolor[HTML]{EEA69F}34 & \cellcolor[HTML]{F6D4D1}65 & \cellcolor[HTML]{F2BCB8}50 & \cellcolor[HTML]{EFADA8}39 & \cellcolor[HTML]{F9E3E1}76 & \cellcolor[HTML]{F2C0BB}52 & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{C2E7D5}97 & \cellcolor[HTML]{BCE4D1}97 & \cellcolor[HTML]{73C79E}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{92D3B3}98  & \cellcolor[HTML]{89D0AD}98 \\
\midrule
XL
    & Top 1\%                        & \cellcolor[HTML]{F5CECA}62                      & \cellcolor[HTML]{F1BAB5}48 & \cellcolor[HTML]{F6D4D1}66 & \cellcolor[HTML]{F6D2CF}64 & \cellcolor[HTML]{F4C7C3}57 & \cellcolor[HTML]{F8DAD7}70 & \cellcolor[HTML]{FAE5E3}77 & \cellcolor[HTML]{F6D0CD}63 & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{8BD1AF}98 & \cellcolor[HTML]{76C8A0}99 & \cellcolor[HTML]{57BB8A}100 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{57BB8A}100 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{6AC397}99 \\
    & 1--10\%                        & \cellcolor[HTML]{F9E3E1}76                      & \cellcolor[HTML]{F4C6C2}56 & \cellcolor[HTML]{F5CFCB}62 & \cellcolor[HTML]{F8DBD9}71 & \cellcolor[HTML]{F3C5C1}55 & \cellcolor[HTML]{F0B2AD}43 & \cellcolor[HTML]{FAE7E5}78 & \cellcolor[HTML]{F6D0CD}63 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{73C79E}99 & \cellcolor[HTML]{6AC397}99 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{6AC397}99 \\
    & 10--20\%                       & \cellcolor[HTML]{FBEBEA}82                      & \cellcolor[HTML]{F4C8C4}57 & \cellcolor[HTML]{F6D0CD}63 & \cellcolor[HTML]{FCF2F2}86 & \cellcolor[HTML]{F4C8C4}58 & \cellcolor[HTML]{EC9D97}29 & \cellcolor[HTML]{FCF2F1}86 & \cellcolor[HTML]{F6D4D1}66 & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{82CDA8}99 & \cellcolor[HTML]{79C9A2}99 & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{70C59B}99 \\
    & 20--30\%                       & \cellcolor[HTML]{FBEBE9}81                      & \cellcolor[HTML]{F4C6C2}56 & \cellcolor[HTML]{F5CCC9}60 & \cellcolor[HTML]{FCF0EF}85 & \cellcolor[HTML]{F4C6C2}56 & \cellcolor[HTML]{F0B4AF}44 & \cellcolor[HTML]{FDF4F3}88 & \cellcolor[HTML]{F7D6D3}67 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{6AC397}99 & \cellcolor[HTML]{7FCCA6}99 & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{6DC49A}99 \\
    & Bottom 50\%                    & \cellcolor[HTML]{FAE5E4}78                      & \cellcolor[HTML]{F3C2BE}54 & \cellcolor[HTML]{F4CAC6}59 & \cellcolor[HTML]{FBEAE9}81 & \cellcolor[HTML]{F5CDCA}61 & \cellcolor[HTML]{F0B5B0}44 & \cellcolor[HTML]{FCF0EF}84 & \cellcolor[HTML]{F6D4D1}66 & \cellcolor[HTML]{57BB8A}100 & \cellcolor[HTML]{7FCCA6}99 & \cellcolor[HTML]{73C79E}99 & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{8ED2B1}98  & \cellcolor[HTML]{71C69C}99 \\
\midrule
XXL
    & Top 1\%                        & \cellcolor[HTML]{F7D8D5}68                      & \cellcolor[HTML]{F5CBC8}60 & \cellcolor[HTML]{FAE5E3}77 & \cellcolor[HTML]{F5CFCC}63 & \cellcolor[HTML]{F8DCD9}71 & \cellcolor[HTML]{F9E3E1}76 & \cellcolor[HTML]{FBEAE8}81 & \cellcolor[HTML]{F8DBD9}71 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{8BD1AF}98 & \cellcolor[HTML]{7CCAA4}99 & \cellcolor[HTML]{7CCAA4}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{98D5B7}98  & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{7BCAA3}99 \\
    & 1--10\%                        & \cellcolor[HTML]{FDF4F4}88                      & \cellcolor[HTML]{F8DFDD}73 & \cellcolor[HTML]{F9E4E2}77 & \cellcolor[HTML]{F9E1DF}74 & \cellcolor[HTML]{F8DDDB}72 & \cellcolor[HTML]{F2BFBA}51 & \cellcolor[HTML]{FAE8E6}79 & \cellcolor[HTML]{F9DFDD}73 & \cellcolor[HTML]{6AC397}99  & \cellcolor[HTML]{7CCAA4}99 & \cellcolor[HTML]{73C79E}99 & \cellcolor[HTML]{79C9A2}99  & \cellcolor[HTML]{82CDA8}99  & \cellcolor[HTML]{61BF91}100 & \cellcolor[HTML]{76C8A0}99  & \cellcolor[HTML]{74C79E}99 \\
    & 10--20\%                       & \cellcolor[HTML]{FEFAFA}92                      & \cellcolor[HTML]{F9E4E2}76 & \cellcolor[HTML]{FAE5E3}77 & \cellcolor[HTML]{FDF8F7}90 & \cellcolor[HTML]{FAE7E5}79 & \cellcolor[HTML]{F0B1AC}42 & \cellcolor[HTML]{FDF6F6}89 & \cellcolor[HTML]{FAE6E4}78 & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{7FCCA6}99 & \cellcolor[HTML]{85CEAA}99 & \cellcolor[HTML]{82CDA8}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{67C295}100 & \cellcolor[HTML]{7FCCA6}99  & \cellcolor[HTML]{77C8A1}99 \\
    & 20--30\%                       & \cellcolor[HTML]{FEFDFD}93                      & \cellcolor[HTML]{F9E0DD}74 & \cellcolor[HTML]{FAE6E4}78 & \cellcolor[HTML]{FDF8F7}90 & \cellcolor[HTML]{FBEAE9}81 & \cellcolor[HTML]{F6D2CF}64 & \cellcolor[HTML]{FDF5F4}88 & \cellcolor[HTML]{FBEBE9}81 & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{8ED2B1}98 & \cellcolor[HTML]{82CDA8}99 & \cellcolor[HTML]{7FCCA6}99  & \cellcolor[HTML]{70C59C}99  & \cellcolor[HTML]{5BBD8D}100 & \cellcolor[HTML]{6DC499}99  & \cellcolor[HTML]{76C89F}99 \\
    & Bottom 50\%                    & \cellcolor[HTML]{FEFCFB}93                      & \cellcolor[HTML]{F8DAD7}70 & \cellcolor[HTML]{FAE5E4}77 & \cellcolor[HTML]{FDF6F6}89 & \cellcolor[HTML]{FBEAE8}80 & \cellcolor[HTML]{F7D9D6}69 & \cellcolor[HTML]{FCF1F0}85 & \cellcolor[HTML]{FBEAE8}80 & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{79C9A2}99 & \cellcolor[HTML]{85CEAA}99 & \cellcolor[HTML]{85CEAA}99  & \cellcolor[HTML]{64C093}100 & \cellcolor[HTML]{5EBE8F}100 & \cellcolor[HTML]{B3E1CA}97  & \cellcolor[HTML]{7AC9A3}99 \\
\bottomrule
\end{tabular}
\caption{WikiSpell exact-match accuracy results on 7 diverse languages. mT5 and ByT5 models (with frozen encoders) were fine-tuned on the combined training sets of all languages.}
\label{tab:wikispell-results-all-langs-full}
\end{table*}



